Correlating Effectiveness of Pointer Analysis Techniques with Patterns in Embedded System Code

A pointer analysis maps the pointers in a program to the memory locations they point to. In this work, we study the effectiveness of the three flavors of pointer analysis namely flow sensitive, flow insensitive, and context sensitive analysis on seven embedded code sets used in the industry. We compare precision gain i.e., the reduction in the number of spurious memory locations pointed by a pointer in each of these settings. We found that in 90% of cases the pointer information was same in all three settings. In other cases, context sensitive analysis was 2.6% more precise than flow sensitive analysis which was 6.8% more precise than flow insensitive analysis on average. We correlate precision gain with coding patterns in the embedded systems-which we believe to be first of its kind activity.

==> defs.tex <==
%
%\usepackage{hyperref} 
\usepackage{pgfplots}
\pgfplotsset{width=12.5cm, height=8cm} 
\usepgfplotslibrary{groupplots}
\usepackage[subnum]{cases}
\usepackage{amsmath}
\usepackage{latexsym}
%\usepackage[table,xcdraw]{xcolor}
\usepackage{booktabs}
\usepackage{comment}
\usepackage{algorithm}
\usepackage{algorithmic}
\usepackage{multirow}
%\usepackage{listings}
%\usepackage{times}

%additonal packages

\usepackage{multido}
\usepackage{paralist}
\usepackage{listings}
\usepackage{color}
\usepackage{comment}
\usepackage{etex}
%for algorithm
\usepackage{algorithm}
\usepackage{algorithmic}
\usepackage{multirow}
%\usepackage[table,xcdraw]{xcolor}
%for textstrikethrough
\usepackage[normalem]{ulem}
\usepackage[makeroom]{cancel}
\usepackage{minibox}
\usepackage{stmaryrd}%added for eval brackets
%\usepackage{amssymb}%for restriction package
\usepackage{wrapfig}%for wrapfig
%\usepackage{soul}
%\usepackage{algpseudocode}
%\usepackage[]{algorithm2e}
%\newcommand*\DNA{\textsc{dna}}

%\newcommand*\Let[2]{\State #1 $\gets$ #2}
%\algrenewcommand\algorithmicrequire{\textbf{Precondition:}}
%\algrenewcommand\algorithmicensure{\textbf{Postcondition:}}
%\newcommand*\Let[2]{\State #1 $\gets$ #2}
%\algrenewcommand\algorithmicrequire{\textbf{Precondition:}}
%\algrenewcommand\algorithmicensure{\textbf{Postcondition:}}
%end for algorithm

\definecolor{dkgreen}{rgb}{0,0.6,0}
\definecolor{gray}{rgb}{0.5,0.5,0.5}
\definecolor{mauve}{rgb}{0.58,0,0.82}

\lstset{frame=tb,
  language=C,
  aboveskip=3mm,
  belowskip=3mm,
  showstringspaces=false,
  columns=flexible,
  basicstyle={\small\ttfamily},
  numbers=left,
  numberstyle=\tiny\color{gray},
  keywordstyle=\color{blue},
  commentstyle=\color{dkgreen},
  stringstyle=\color{mauve},
  breaklines=true,
  breakatwhitespace=true,
  tabsize=3
}
\usepackage{pstricks}
\usepackage{pst-node}
\usepackage{pst-blur}
\usepackage{pst-rel-points}
\usepackage{xspace}


%end additional packages
%graph
\usepackage{pgfplots, pgfplotstable}
\usepackage{tikz}
\usetikzlibrary{patterns}
\usepackage{url}
\usepackage[normalem]{ulem}
%\usepackage{amsthm}

\newrgbcolor{brown}{.65 0.15 .0}
\newrgbcolor{violet}{.84 0 .96}
\newrgbcolor{mygreen}{.24 .84 .72}

\newcommand{\UKcomment}[1]{{\brown [\protect#1 (Uday)]}}
\newcommand{\UKadd}[1]{{\blue \protect#1}}
\newcommand{\UKdel}[1]{{\green \protect#1}}
\newcommand{\UKchange}[2]{\UKadd{\protect#1} {\brown[Was: {\green\protect#2}]}}

\newcommand{\KPcomment}[1]{{\red \protect#1 (Komal)}}
\newcommand{\KPadd}[1]{{\cyan \protect#1}}
\newcommand{\KPdel}[1]{{\magenta was: \protect#1}}
\newcommand{\mofp}{\text{MoFP}\xspace}
\newcommand{\mfp}{\text{MFP}\xspace}
\newcommand{\mop}{\text{MoP}\xspace}
\newcommand{\ppmfp}{\text{PPMFP}\xspace}
\newcommand{\FI}{\text{FI}\xspace}
\newcommand{\cfg}{\text{CFG}\xspace}

\newcommand{\cstart}{\text{$\mathcal{C}(start,e)$}\xspace}
\newcommand{\cend}{\text{$\mathcal{C}(end,e)$}\xspace}
\newcommand{\negcend}{\text{$\mathcal{C}(\neg end,e)$}\xspace}
\newcommand{\bvalREnd}{\text{$\overline{X}\!\mid_{\neg\cend}$}\xspace}



\psset{unit=1mm}


\newcommand{\add}{\blue}
\newcommand{\delete}{\green}
\newcommand{\colort}{\red}
%\newcommand{\note}{\red Note: }
%\newcommand{\cfp}{\text{$\rho$}\xspace}
%\newcommand{\cfpmips}{\text{$\rho_1'$}\xspace}

\newcommand{\mips}{\text{MIPS}\xspace}
\newcommand{\cfp}{\text{CFP}\xspace}
\newcommand{\cfps}{\text{{CFP\/}s}\xspace}
\newcommand{\paths}{\text{\em paths}\xspace}
\newcommand{\cpaths}{\text{\em cpaths}\xspace}
\newcommand{\prefixes}{\text{\em prefixes}\xspace}
\newcommand{\symmips}{\text{$\mu$}\xspace}
\newcommand{\dfv}{\text{$\delta$}\xspace}
\newcommand{\setmips}{\text{\em M}\xspace}
\newcommand{\nd}{\text{\em end}\xspace}
%\newcommand{\cmips}{\text{\em cmips}\xspace}
\newcommand{\cmips}{\text{cluster}\xspace}
\newcommand{\cmipss}{\text{clusters}\xspace}
\newcommand{\ips}{\text{\em ips}\xspace}

\newcommand{\onetb}{\ \ \ }
\newcommand{\twotb}{\ \ \ \ \ \ }
\newcommand{\threetb}{\ \ \ \ \ \ \ \ \ }
\newcommand{\fourtb}{\ \ \ \ \ \ \ \ \ \ \ \ }

\newcommand{\ao}{$a_{n1}$}
\newcommand{\at}{$a_{n4}$}
\newcommand{\bo}{$b_{n1}$}
\newcommand{\bt}{$b_{n3}$}
\newcommand{\aobo}{\{\ao,\bo\}}
\newcommand{\aobt}{\{\ao,\bt\}}
\newcommand{\atbt}{\{\at,\bt\}}
\newcommand{\ab}{\{\ao,\bo,\at,\bt\}}
\newcommand{\emty}{\{\} }

\newcommand{\dzero}{$d_0$}
\newcommand{\dsix}{\text{$d_{e6}$}}

\newcommand{\INDSTATE}[1][1]{\STATE\hspace{#1\algorithmicindent}}

\newcommand{\ps}{\text{$\rho$}}
\newcommand{\elab}{\text{\em label}\xspace}
\newcommand{\cond}{\text{\em cond}\xspace}
\newcommand{\vars}{\text{\em vars}\xspace}
\newcommand{\true}{\text{\em true}\xspace}
\newcommand{\false}{\text{\em false}\xspace}
\newcommand{\block}{\text{\em blocks}\xspace}
\newcommand{\unknown}{\text{\em unknown}\xspace}
\newcommand{\eval}[2]{\text{$\llbracket \protect #1 \rrbracket_{#2}$}\xspace}
\newcommand{\states}[2]{\text{\emph{states}$(\protect #1, \protect#2)$}\xspace}

\newcommand{\meet}{\text{$\;\sqcap\;$}}
\newcommand{\cmfp}{\text{$\llbracket MFP \rrbracket_s$}\xspace}
\newcommand{\cmfps}[1]{\text{$\llbracket MFP \rrbracket_{\protect#1}$}\xspace}
\newcommand{\confined}{\emph{confined }}
\newcommand{\pp}{\emph{partially path-sensitive}\xspace}
\newcommand{\mtext}[1]{\text{$\protect #1$}\xspace}
\newcommand{\xmap}[1]{x\text{$\mapsto$}\protect#1}
\newcommand{\es}{\emph{s}\xspace}
\newcommand{\mipsstart}{\emph{start}\xspace}
\newcommand{\mipsend}{\emph{end}\xspace}
\newcommand{\mipsinner}{\emph{inner}\xspace}
\newcommand{\mipsfront}{\emph{frontier}\xspace}
\newcommand{\cluster}{\emph{cluster}\xspace}
\newcommand{\symcluster}{\emph{$\psi$}\xspace}
\newcommand{\clusters}{\emph{clusters}\xspace}
\newcommand{\Pred}{\emph{pred}\xspace}
\newcommand{\Succ}{\emph{succ}\xspace}
\newcommand{\Boundary}{\emph{\sffamily BI}\xspace}
\newcommand{\Start}{\emph{\sffamily Start}\xspace}
\newcommand{\End}{\emph{\sffamily End}\xspace}
\newcommand{\Out}{\emph{\sffamily Out}\xspace}
\newcommand{\In}{\emph{\sffamily In}\xspace}
\newcommand{\bOut}{\text{$\overline{\emph{\sffamily Out}}$}\xspace}
\newcommand{\bIn}{\text{$\overline{\emph{\sffamily In}}$}\xspace}
\newcommand{\hlat}{\text{$\widehat{L}$}\xspace}
\newcommand{\blat}{\text{$\overline{L}$}\xspace}
\newcommand{\bval}{\text{$\overline{X}$}\xspace}
\newcommand{\bvalR}{\text{$\overline{X}\!\mid_s$}\xspace}
\newcommand{\lat}{\text{$L$}\xspace}
\newcommand{\pOut}{\text{$\overline{\overline{\emph{\sffamily Out}}}$}\xspace}
\newcommand{\pIn}{\text{$\overline{\overline{\emph{\sffamily In}}}$}\xspace}

\newcommand{\zero}{\texttt{$l\!\mapsto\! [0,0]$}}
\newcommand{\one}{\texttt{$l\!\mapsto\! [1,1]$}}
\newcommand{\zeroone}{\texttt{$l\!\mapsto\! [0,1]$}}

\newcommand{\lzero}{\texttt{$l\!\mapsto\!0$}}
\newcommand{\lone}{\texttt{$l\!\mapsto\!1$}}
%\newcommand{\dfi}[2]{\minibox{$d_1:\protect #1$\\$d_2:\protect #2$}}
\newcommand{\dfi}[2]{\minibox{$\left\langle \protect #1, \protect #2\right\rangle$}}
\def\duline#1{\underline{\underline{#1}}}
\newcommand{\result}[3]{\underline{$R[e_#1,q_{e#2}]$ = #3 }}
\newcommand{\q}[1]{q_{e#1}}
\newcommand{\visited}[2]{\underline{$V[e_#1]=\{#2\}$}}
	
	
\newcommand{\bBoundary}{\text{$\overline{\emph{\sffamily BI}}$}\xspace}
\newcommand{\bG}{\text{$\overline{\emph{\sffamily g}}$}\xspace}
\newcommand{\bgnoarg}{\text{$\emph{\sffamily g}$}\xspace}
\newcommand{\bg}[1]{\text{$g_{m\rightarrow n}(\protect #1)$}\xspace}
\newcommand{\bF}{\text{$\overline{f}$}\xspace}
\newcommand{\bMeet}{\text{\;$\overline{\sqcap}$\;}\xspace}
\newcommand{\edgee}{\text{e}\xspace}
\newcommand{\mipsunmarked}{\text{unmarked}\xspace}
\newcommand{\di}{\text{$d_i$}\xspace}
\newcommand{\dni}[1]{\text{$d_i^{#1}$}\xspace}
\newcommand{\ditwo}{\text{$d_i'$}\xspace}
\newcommand{\dilast}{\text{$d_{k+1}$}\xspace}
\newcommand{\dnilast}[1]{\text{$d_{k+1^{#1}}$}\xspace}
\newcommand{\dilasttwo}{\text{$d_{k+1}'$}\xspace}
\newcommand{\clusteri}{\text{$\symcluster_i$}\xspace}
\newcommand{\clusterj}{\text{$\symcluster_j$}\xspace}
\newcommand{\mipsi}{\text{$\symmips_i$}\xspace}
\newcommand{\mipsj}{\text{$\symmips_j$}\xspace}
\newcommand{\coment}[2]{\protect #1\text{ \emph{\protect #2}}\xspace\\}
\newcommand{\pMeet}{$\bigsqcap\limits_{1\leq i\leq k+1} d_i$}
\newcommand{\dtuple}{\text{\angles{d_1,d_2,\ldots,d_{k+1}}}\xspace}
\newcommand{\dntuple}[1]{\text{\angles{d_1^{#1},d_2^{#1},\ldots,d_{k+1}^{#1}}}\xspace}
\newcommand{\dtupletwo}{\text{\angles{d_1',d_2',\ldots,d_{k+1}'}}\xspace}
\newcommand{\angles}[1]{\text{$\langle\protect #1\rangle$}}
\newcommand{\mn}{\text{$m \rightarrow n$}\xspace}
\newcommand{\no}{\text{$n \rightarrow o$}\xspace}
\newcommand{\bGmn}[2]{\text{$\bG_{\protect #1\rightarrow \protect #2}$}}
\newcommand{\bGe}{\text{$\overline{g}_e$}}
\newcommand{\bGei}[1]{\text{$\overline{g}_e^{#1}$}}
\newcommand{\Ge}{\text{$g_e$}}

\newcommand{\rangeZT}{\text{$l\mapsto[0,2]$}\rule[-5pt]{0em}{15pt}\xspace}
\newcommand{\rangeZ}{\text{$l\mapsto[0,0]$}\rule[-5pt]{0em}{15pt}\xspace}
\newcommand{\rangeT}{\text{$l\mapsto[2,2]$}\rule[-5pt]{0em}{15pt}\xspace}
\newcommand{\rangeTop}{\text{$l\mapsto[+\infty,-\infty]$}\rule[-5pt]{0em}{15pt}\xspace}
\newcommand{\setZT}{\text{$l\mapsto\{0,2\}$}\rule[-5pt]{0em}{15pt}\xspace}
\newcommand{\setZ}{\text{$l\mapsto\{0\}$}\rule[-5pt]{0em}{15pt}\xspace}
\newcommand{\setT}{\text{$l\mapsto\{2\}$}\rule[-5pt]{0em}{15pt}\xspace}

\newcommand{\crangeZT}{\text{$c\mapsto[0,2]$}\rule[-5pt]{0em}{15pt}\xspace}
\newcommand{\crangeZ}{\text{$c\mapsto[0,0]$}\rule[-5pt]{0em}{15pt}\xspace}
\newcommand{\crangeT}{\text{$c\mapsto[2,2]$}\rule[-5pt]{0em}{15pt}\xspace}
\newcommand{\crangeTop}{\text{$c\mapsto[+\infty,-\infty]$}\rule[-5pt]{0em}{15pt}\xspace}

\newcommand{\same}{*}
%\newcommand{\setof}[1]{\{#1\}}
\newcommand{\pair}[1]{\langle #1 \rangle}

\newcommand{\mipss}{\text{MIPSs}\xspace}


\newcommand{\mstart}{\mipsstart(\symmips)}
\newcommand{\minner}{\mipsinner(\symmips)}
\newcommand{\mend}{\mipsend(\symmips)}

\newcommand{\bblat}{\text{$\overline{\lat}$}\xspace}
\newcommand{\bbIn}{\text{$\overline{\overline{In}}$}}
\newcommand{\bbbIn}{\text{$\overline{\bbIn}$}}

\newcommand{\bbOut}{\text{$\overline{\overline{Out}}$}}
\newcommand{\bbbOut}{\text{$\overline{\bbOut}$}}

\newcommand{\bbF}{\text{$\overline{\overline{F}}$}}
\newcommand{\bbBoundary}{\text{$\overline{\bBoundary}$}}
\newcommand{\bbMeet}{\text{$\overline{\overline{\bigsqcap}}$}}
\newcommand{\bbMeets}{\text{$\overline{\overline{\sqcap}}$}}
\newcommand{\sdash}{\text{$S'$}}
\newcommand{\sddash}{\text{$S''$}}
\newcommand{\lvalue}[2]{\{\text{$\langle$}\protect #1,\protect #2\text{$\rangle$}\}}
\newcommand{\set}[1]{\{\protect #1\}}
\newcommand{\tinyset}[1]{\{\protect #1\}}
\newcommand{\foldmeet}{\text{$fold_{\sqcap}$}}
\newcommand{\update}{attach}
\newcommand{\val}{\text{$\Pi$}}
\newcommand{\project}[2]{\text{\ensuremath{\pi_{#1}^{#2}}}}
\newcommand{\merg}{add}
\newcommand{\sinner}{\emph{live} }
\newcommand{\tentb}{\fourtb\fourtb\twotb}

\newcommand{\btop}{\text{$\overline{\top}$}}
\newcommand{\bbtop}{\text{$\overline{\btop}$}}
\newcommand{\default}{\emph{default} }
\newcommand{\powerset}[1]{\text{$\mathcal{P}(#1)$}}

\newcommand{\mpowerset}{\text{$\mathcal{P}(\setmips)$}}
\newcommand{\lpowerset}{\text{$\mathcal{P}(\hlat)$}}
\newcommand{\fun}{\text{\em f} }
\newcommand{\fune}{\text{\em g} }
\newcommand{\property}{\text{\em PresP} }
\newcommand{\propertyr}{\text{$\nabla\property$} }

